Aryl: An Elastic Cluster Scheduler for Deep Learning

Companies build separate training and inference GPU clusters for deep learning, and use separate schedulers to manage them. This leads to problems for both training and inference: inference clusters have low GPU utilization when the traffic load is low; training jobs often experience long queueing time due to lack of resources. We introduce Aryl, a new cluster scheduler to address these problems. Aryl introduces capacity loaning to loan idle inference GPU servers for training jobs. It further exploits elastic scaling that scales a training job's GPU allocation to better utilize loaned resources. Capacity loaning and elastic scaling create new challenges to cluster management. When the loaned servers need to be returned, we need to minimize the number of job preemptions; when more GPUs become available, we need to allocate them to elastic jobs and minimize the job completion time (JCT). Aryl addresses these combinatorial problems using principled heuristics. It introduces the notion of server preemption cost which it greedily reduces during server reclaiming. It further relies on the JCT reduction value defined for each additional worker for an elastic job to solve the scheduling problem as a multiple-choice knapsack problem. Prototype implementation on a 64-GPU testbed and large-scale simulation with 15-day traces of over 50,000 production jobs show that Aryl brings 1.53x and 1.50x reductions in average queuing time and JCT, and improves cluster usage by up to 26.9% over the cluster scheduler without capacity loaning or elastic scaling.

==> future.tex <==
%!TEX root = main.tex

\section{Future work}
\label{sec:future_work}

The future work part.

==> highlight.tex <==
%!TEX root = main.tex

\section{Design Philosophy}
\label{sec:choices}

The highlight part.




==> overview.tex <==
%!TEX root = main.tex

\section{Overview}
\label{sec:Overview}
We plan to extend this different aspects. First, we will implement NetKernel in linux kernel to improve the efficiency. Second, more NSM images will be fostered, including different transport-protocols (e.g. DCTCP, RDMA), OS optimizations, and network functions. Finally, we will experiment NetKernel in more complex environments.

